Modeling Human Annotation Errors to Design Bias-Aware Systems for Social Stream Processing

High-quality human annotations are necessary to create effective machine learning systems for social media. Low-quality human annotations indirectly contribute to the creation of inaccurate or biased learning systems. We show that human annotation quality is dependent on the ordering of instances shown to annotators (referred as 'annotation schedule'), and can be improved by local changes in the instance ordering provided to the annotators, yielding a more accurate annotation of the data stream for efficient real-time social media analytics. We propose an error-mitigating active learning algorithm that is robust with respect to some cases of human errors when deciding an annotation schedule. We validate the human error model and evaluate the proposed algorithm against strong baselines by experimenting on classification tasks of relevant social media posts during crises. According to these experiments, considering the order in which data instances are presented to human annotators leads to both an increase in accuracy for machine learning and awareness toward some potential biases in human learning that may affect the automated classifier.

==> 02-background.tex <==
%!TEX root = main.tex

\section{Background}\label{sec:background}

\subsection{Online active learning}  
Existing types of online active learning methods, to the best of our knowledge, address only possible machine biases and errors.  
% 
Gama et al.~\cite{gama2014survey} and Almeida et al.~\cite{almeida2018adapting} provide an extensive survey of the different active learning methods. The primary categories for the active learning methods include one group focused on better sampling of the instance space for querying (e.g., addressing concept drift~\cite{zliobaite2014active}), and another group focused on better learning of a discriminatory model.        
% 
However, our research premise is that the improvement of both of the above active learning methods for stream processing systems requires to account the mitigation for the potential oracle/human errors during querying as well, in order to be both efficient and unbiased in the modeling.  

% \begin{table*}[ht!]
% \small
% \caption{Framework of human annotation errors in stream processing systems. (*\textit{primary focus of our experiments}) 
% \label{tbl:human-errors-framework}}
%     \begin{tabular}{%p{1in}
% 							p{2.0in}p{2.3in}p{2.3in}} 
% 	   \toprule
%       % \multicolumn{1}{l}{\textbf{Main cause}} &
%         \multicolumn{1}{c}{\textbf{Type of Error}} & 
%         \multicolumn{1}{c}{\textbf{Potential Cause}} & 
%         \multicolumn{1}{c}{\textbf{Mitigation Approach}} 
%         \\ 
%         \midrule
%         %\begin{minipage}[b][1\baselineskip][c]{1in}
%         %\textbf{\mbox{Time constraints}}
%         %\end{minipage} &
%         \begin{minipage}[c][1\baselineskip][t]{1.3in}
%           \mbox{ %\refhypothesis{h:slips-time}. 
%           Slips induced by %} \mbox{
%           time constraints}
%         \end{minipage} &
%         \begin{minipage}[c][1\baselineskip][t]{2.3in}
%             \begin{itemize} %{compactenum}[1.]
%                 %%\item[\ref{e:fatigue}.] Slips due to fatigue
%                 %%\item[\ref{e:time-pressure}.] Slips due to time pressure
%                 \item%[\ref{e:concept-forgotten}.] 
%                       Concept forgotten 
%             \end{itemize} %{compactenum}
%         \end{minipage} &
%         \begin{minipage}[c][1\baselineskip][t]{2.3in}
%             \begin{itemize} %{compactenum}[1.]
%                 %%\item Limit annotation volume
%                 %%\item Limit annotation velocity
%                 \item Show reminder for concept examples
%             \end{itemize} %{compactenum} 
%         \end{minipage}
%         \\ 
%         \midrule 
%         %%\multirow{1}{*}{
%         %\begin{minipage}[c][1\baselineskip][c]{1in}
%         %\textbf{\mbox{Serial ordering}}
%         %\end{minipage}
%         %%}  &
%         \begin{minipage}[c][1\baselineskip][t]{1.3in}
%         \mbox{ %\refhypothesis{h:ordering-mistakes}: 
%         \textit{* Mistakes induced by %} \mbox{
%         serial ordering}}
%         \end{minipage} &
%         \begin{minipage}[c][1\baselineskip][t]{2.3in}
%             \begin{itemize} %{compactenum}[1.]
%                 \item %[\ref{e:concept-not-acquired}.] 
%                         Concept not acquired yet or forgotten
%             \end{itemize} %{compactenum}
%         \end{minipage} &
%         \begin{minipage}[c][1\baselineskip][t]{2.3in}
%             \begin{itemize} %{compactenum}[1.]\setcounter{enumi}{2}
%                 \item Show frequent learning examples
%             \end{itemize} %{compactenum}
%         \end{minipage}
%         \\
%          \midrule 
%          \begin{minipage}[c][2\baselineskip][t]{1.3in}
%          \mbox{ %\refhypothesis{h:ordering-slips}: 
%          \textit{* Slips induced by %} \mbox{
%          serial ordering}}
%          \end{minipage} &
%          \begin{minipage}[c][2\baselineskip][t]{2.3in}
%              \begin{itemize} %{compactenum}[1.]
%                  \item %[\ref{e:high-availability}.] 
%                       Presence of a high-availability concept or
%                       a low-availability concept
%              \end{itemize} %{compactenum}
%          \end{minipage} &
%          \begin{minipage}[c][2\baselineskip][t]{2.5in}
%              \begin{itemize} %{compactenum}[1.]\setcounter{enumi}{5}
%                  \item Limit extreme divergence from base rate
%              \end{itemize} %{compactenum}
%          \end{minipage}
%          \\
%         \bottomrule
%     \end{tabular}
% \vspace{-0.2in}
% \end{table*}

% \subsection{Human annotator biases}

% Annotation quality can be affected by many factors. 
% %
% The nature of the annotation task is perhaps the most obvious one, with some tasks being inherently easier than others. For instance, guessing the gender of a person given a photo is easier than guessing his/her age~\cite{nguyen2014gender}.
% %
% The skewness of the distribution of classes is another problem in the annotation tasks. Especially, the tasks in which the dominant class is too prevalent lead to difficulties in appropriately representing the minority class for helping human annotators learn the minority class concepts~\cite{cohen2013classifying}.   
% %
% Annotation styles are also known to affect human annotation quality with respect to factors such as objectivity and  descriptiveness~\cite{cheng2013annotation}. 
% %
% % Prior literature~\cite{zhang2004cognitive} based on Reasons' error taxonomy~\cite{reason1990human} indicate a popular classification of errors into \textit{mistakes} and \textit{slips}, which can be also classified as execution or evaluation errors. 
% % %Chronological bias~\cite{pannucci2010identifying} is the confounding of time, e.g., differences between those recruited early or later in a study, or a tendency to use historical information when more recent samples should be given more importance.
% % %
% % Additionally, studies in the prior literature also point to the other factors for human errors, such as cognitive biases in the annotation task design~\cite{burghardt2018quantifying} and recency effects(e.g., ~\cite{seufert2016one} shows that after watching a high-quality video user judgment become more extreme and then, users judged as much lower quality the low-quality videos and as much higher quality the high-quality videos.)  
% % 
% Furthermore, annotation expertise affects quality, particularly in difficult tasks~\cite{hansen2013quality} as well as the cognitive biases in the annotation task design sometimes lead to human errors~\cite{burghardt2018quantifying}. 
% %
% Thus, there is a need to systematically develop a framework to organize and investigate specific human error types in the annotation tasks of HSPS. 

%\subsection{Algorithmic biases}
%Algo. Bias modeling in general \\ 
%... (strategies to mitigate biases) ... \\ 

%\todo{pros and cons of three experiment types}

==> 03-human-annotation.tex <==
%!TEX root = main.tex

\section{Human Annotation Error Modeling}\label{sec:human-errors}

In this section we present qualitative %and quantitative 
evidence on the human biases that lead to potential annotation errors. 

\spara{Assumptions.}  
We assume that the cognitive representation of the concept (e.g., reports of infrastructure damage during a disaster) at the beginning of the annotation task is only partial, in the sense that the boundaries and the nuances about a concept are learned while the annotations are performed. 
We also assume that the annotator can develop a cognitive representation of a concept by seeing a sufficient number of examples of this concept, even if the examples are not annotated a priori, which is usually the case. 

\spara{Errors.} 
Following the highly cited psychology study of human error taxonomy by Reasons~\cite{reason1990human} and medical domain errors~\cite{zhang2004cognitive}, %as well as the associated references therein, 
we distinguish two classes of errors: \textit{mistakes} and \textit{slips}. 
\emph{Mistakes} are caused by not acquiring the correct cognitive representation of a concept. 
\emph{Slips} are errors that happen despite acquiring the correct cognitive representation of a concept. 

% Based on these broad classes, %section~\ref{subsec:human-errors-framework} presents 
% we present a taxonomy of human errors in stream processing in Table~\ref{tbl:human-errors-framework} and explain the main error types below. 
% %During the exposition of this taxonomy, 
% We do not claim that all classes of human errors are equally prevalent or are equally severe.  
% %
% %Section~\ref{sec:human-errors-experiments} describes how to measure experimentally the prevalence and severity of the different classes of errors, and Section~\ref{subsec:human-errors-results} presents the crowdsourcing experiment results. 
% %
% %\subsection{Error Model of Stream Annotation}\label{subsec:human-errors-framework}
% %
% %%%%%%%%%%%
% % In particular, we identify two primary ways in which the characteristics of a stream annotation task can induce human error: %\\ %\begin{inparaenum}[(i)]
% % %\item slips due to time constraints,
% % a.) Slips due to time constraints or serial ordering, and %\\ 
% % b.) Mistakes due to serial ordering.  %\\ 
% %%%%%%%%%%%
% %end{inparaenum}
% %
% %Table~\ref{tbl:human-errors-framework} summarizes this error typology. 
% %, which are explained next. % using the hypothesis statements.

% % %%%%%%%%%%%
% % %\mpara{\newhypothesis{h:slips-time}. Time constraints induce slips.}
% % \subsubsection{Time Constraint-induced Slips} 
% % %%%%%%%%%%%
% % The necessity to label many elements in a short period of time, i.e., the volume and the velocity of the stream compared to human capacity to annotate, may cause \emph{slips}; the annotator could a correct representation of a concept, but fails to apply it. 
% % %
% % We consider two types of slips caused by temporal constraints:

% % \begin{itemize} %{compactenum}[1.]
% %     \item\label{e:fatigue} Slips due to fatigue after having labeled a large number of items, which translate into burnout: a reduction in annotation quality.
% %     \item\label{e:time-pressure} Slips due to time pressure when applying a complex concepts, i.e., when the annotation of an item requires more time than what the annotator would/could allocate.
% % \end{itemize} %{compactenum}

% % \noindent
% % In the first case, the solution is to limit the maximum number of annotations tasks required by an annotator, and to include rest periods. 
% % %
% % In the second case, the solution is to limit the rate at which the annotator is required to label items. 
% % %
% % In general, this type of slip can be managed by imposing an appropriate limit, i.e., a \emph{budget} of annotations per time period. 

% % Slips induced by time constraints %(\textbf{\refhypothesis{h:slips-time}})} 
% % are well established in the psychology literature, with substantive research studying the effect on attention and complex reasoning of fatigue (e.g., \cite{lorist2005impaired,boksem2006mental,van2006mental})
% % % 
% % and time pressure, where speed/accuracy trade-offs are well known (e.g.,~\cite{wickelgren1977speed}) and have even been studied in the specific context of crowdsourcing~\cite{cheng2015measuring}.
% % % 
% % Hence, we focus our attention in the remaining types of errors. %Given the known challenge of cognitive load~\cite{burghardt2018quantifying} for this error type, we chose to skip this in our crowdsourcing experiments and rather, focused on serial ordering effects as detailed next.  

% %%%%%%%%%%%
% % \mpara{\newhypothesis{h:ordering-slips}. Serial ordering induces slips.}
% \subsubsection{Serial Ordering-induced Slips} 
% %%%%%%%%%%%
%  The ordering in which tasks are presented to an annotator may also cause \emph{slips}, in which the annotator erroneously labels an instance even if s/he has a correct representation of its concept.
% %
% We identify two main cases for this type of slip:
% \begin{itemize} %{compactenum}[1.]\setcounter{enumi}{4}
%     \item\label{e:high-availability} Slip towards a concept that is highly available. 
%     %
%     In this case, the annotator is inattentive and erroneously labels an instance with a label that comes easily to his/her mind.
%     %
%     This may be caused by serial position effects~\cite{murdock1962serial} including primacy (a tendency to remember the beginning instances more in the stream) and recency (a tendency to remember the latest instances more), or by having too many instances of the same type (noise w.r.t. a signal) shown in sequence, displacing the other types of instances.  
%     \item\label{e:low-availability} Slip against a concept that is minimally available. 
%     %
%     In this case, the correct category does not come easily to the annotator's mind, because its frequency is too small compared to other categories.
%     %
%     The annotator has not forgotten the concept, s/he is just inattentive and uses a more available label instead of the correct one.
% \end{itemize} %{compactenum}

% Both cases can be seen as problems caused by an extreme local divergence from the base rate or forgetting behavior.  
% %
% These can be prevented by proper annotation schedules. % ordering of instances to avoid local concentration/dilution of a class.

% %%%%%%%%%%%
% %\mpara{\newhypothesis{h:ordering-mistakes}. Serial ordering induces mistakes.}
% \subsubsection{Serial Ordering-induced Mistakes} 
% %%%%%%%%%%%
% The ordering in which the tasks are presented to an annotator may prevent the annotator from adequately understanding a concept, hence introducing \emph{mistakes}. 
% %
% %We identify the following  %two main cases of this 
% The main type of mistake includes:
% \begin{itemize} %{compactenum}[1.]\setcounter{enumi}{2}
%     \item\label{e:concept-not-acquired} Concept not acquired yet or forgotten: The annotator is asked to annotate an instance of a class for which s/he has not seen a sufficient number of examples to learn the concept overall, or recently no examples are shown, which cause him/her errors in the annotation. %covering different sub-classes, which means s/he will only be able to use the definitions given at the beginning of the task, i.e. partial knowledge. %which only partially convey the concept of this class.
%     %\item\label{e:concept-forgotten} Concept forgotten: the annotator is asked to annotate an item for a class for which s/he has not seen \emph{recently} a sufficient number of example, and hence may have forgotten the concept. Recency in this case can be measured in time units, or in number of items annotated since last seeing a concept.
% \end{itemize} %{compactenum}

% %In the first and second cases, m
% Mistakes can be reduced if the ordering of instances in a task 
% is such that a sufficient number of examples of each concept are presented %(\emph{learning} examples), 
% and occasionally some reminders from old concepts, so the annotator does not forget them.  %(\emph{reminder} examples). 

% In the following sections, we present three different approaches to validate the existence of human errors and reason about an algorithmic solution to mitigate these errors: lab-based, crowdsourcing-based, and simulation-based.  
% %
% The lab-based error testing approach is similar to the experiments in psychology, with greater control of the environment for the human annotation task; however, it is difficult to scale to multiple annotators. As a solution, the crowdsourcing-based approach can help to remedy the scalability challenge of the experimental setup, however, it provides less control on the setup to capture the behavior resulting from the unacquired knowledge of the human annotator. Lastly, the simulation-based approach allows us to generate any choice of the streaming data samples, emulate human errors through an automated oracle, and demonstrate error mitigation techniques.  


 

==> 06-crowd-experiment.tex <==

\section{Crowd-scale Annotation Error Testing}\label{sec:human-errors-experiments}

\begin{table*}[ht!]
\caption{Annotation errors in the three positions of the target class message (see text), observed after 120 crowdsourced responses on two types of annotation schedule. The $p$-value indicates the statistical significance for the difference between the error at the third studied position in comparison to the union of the errors at first and second studied positions.   
 \label{tbl:crowd}}
\centering
\begin{tabular}{p{1in}p{1.5in}lllp{0.5in}}
\toprule 
\textbf{Error Type} & \textbf{Potential Cause}   &  \textbf{$1^{st}$ Position Error} & \textbf{$2^{nd}$ Position Error} & \textbf{$3^{rd}$ Position Error} & \textbf{$p$-value} \\
\midrule 
Slip                & forgotten knowledge  & 0.3                      & 0.23                     & 0.32                     & 0.005            \\
Mistake             & unacquired knowledge & 0.27                     & 0.38                     & 0.28                     & 0.11         \\    
\bottomrule 
\end{tabular}
\end{table*}

Our crowd experiments seek to measure the severity of each error and the conditions under which it appears. The goal of these crowd experiments is to establish a motivational foundation %these measurements as inputs 
to design algorithms seeking to--among other goals--minimize these errors. 
%
%Given that these effects might be domain-dependent, we characterize them %within two specific domains: 
%for categorizing emergency-related social media messages. %, and categorizing images.

%Most of the results we present are averaged across users, tasks, and/or classes of messages. 
%In our experiments we bound the time required to perform the task. This is done because given an unlimited amount of time, which is not realistic in our scenario, annotators could trade off more time to completion by more accuracy. 
Specifically, we generated two types of %instance ordering (sequences)
annotation schedule (instance sequence) for the task described in section~\ref{sec:task}, corresponding to mistakes and slips. %to categorize a tweet item into four classes. 
For practical reasons of the cost and time of crowdsourcing, we limited the length of the schedules to 20 instances.   %, as shown in figure~\ref{fig:sequences}.   
% 
For constructing the schedules, we used the labeled data %described in section~\ref{sec:task}
as the ground truth and based on the labeled data distribution, we chose the minority class $c3$ (messages about ``affected individuals'') as our target class for the error analysis.  
%
%The two annotation schedules are expected to capture the error types of mistakes and slips for a target class due to serial ordering respectively, where  %Figure~\ref{fig:sequences} shows the two corresponding sequences. 
%the first schedule is $\{c4,c1,c2,\textit{\textbf{c3}},c1,\textit{\textbf{c3}},c4,c1,c4,c1,c4,c2,c1,c4,c1,c2,c4,c2,c4,\textit{\textbf{c3}}\}$ and the second schedule is $\{c4,c1,c2,c1,c4,c2,c1,c4,\textit{\textbf{c3}},c1,c2,c4,\textit{\textbf{c3}},c1,c2,c1,\textit{\textbf{c3}},c2,c4,c4\}$. 

For studying slips induced by serial ordering, we study the case when tweet instances of a target class ($c3$) are positioned with a mix of short and long gaps in an annotation schedule. We assume that the non-uniform and infrequent occurrences cause the annotators to forget the knowledge of the target class. Thus, we hypothesis that the annotation error per position of the target class should increase at the end of the annotation schedule. 
%
Similarly, we study mistakes induced by serial ordering in the case when tweet instances of a target class ($c3$) are positioned with equal gaps in an annotation schedule. We observe the annotation error at each position in the schedule where an instance of the target class appears. We permute the instances of the target class on these positions. We hypothesize that the uniform and frequent occurrences would allow the annotators to slowly acquire the knowledge of the target class. Thus, we hypothesize that the annotation error per position of the target class should reduce as we move toward the end of the annotation schedule. 

The first annotation schedule corresponding to slip errors is $\{c4$, $c1$, $c2$, $\underline{\textbf{c3}}$, $c1$, $\underline{\textbf{c3}}$, $c4$, $c1$, $c4$, $c1$, $c4$, $c2$, $c1$, $c4$, $c1$, $c2$, $c4$, $c2$, $c4$, $\underline{\textbf{c3}}\}$ and the second schedule corresponding to mistake errors is $\{c4$, $c1$, $c2$, $c1$, $c4$, $c2$, $c1$, $c4$, $\underline{\textbf{c3}}$, $c1$, $c2$, $c4$, $\underline{\textbf{c3}}$, $c1$, $c2$, $c1$, $\underline{\textbf{c3}}$, $c2$, $c4$, $c4\}$. 
%
The underlined class label indicates the target class for analysis. 
% 
For the 3 positions of the target class ($c3$) in an annotation schedule, we permuted the messages shown in those positions, leading to 6 experimental cases for each type of schedule. Each sequence of messages was annotated by 10 human judges using the \textit{Figure Eight} (https://www.figure-eight.com/) platform. In total, we received responses from 120 human judges for the two schedules. 
% 
%First, by considering the learning curve of annotators, i.e., the increase in their accuracy with respect to a class, as a function of the number of examples seen of that class~(as observed by, e.g., \cite{hansen2013quality}). 
%
%Second, by considering the forgetting curve~\cite{averell2011form} of annotators, i.e., the decrease in their accuracy with respect to a class, as a function of the time elapsed since the last example of that class was shown.

%\spara{
%Slips induced by serial ordering %(\textbf{\refhypothesis{h:ordering-slips}})} are also studied by introducing large local discrepancies with the base rate of a class. 
%
%This is done by measuring annotator accuracy in situations in which a class locally (i.e., in a part of the sequence of tasks shown to a user) has highly increased or highly reduced prevalence with respect to its base rate.


\spara{Crowd Annotation Results.} %\label{subsec:human-errors-results}
%In our experiments we control fatigue and time pressure by bounding the total number of tasks and the total time required for each task. 
We analyzed the responses on both types of annotation schedules. Table~\ref{tbl:crowd} shows the results of the crowdsourcing for the micro-average error rate at the positions of the target class in the schedule. We also ran a two-tailed test to observe any statistically significant difference between the errors of the specific positions. 
%
We found a highly significant difference ($p$-value of 0.005) for the error between the last position and the average of the earlier two positions in a sequence that depicts slips due to potentially forgetting the knowledge of the target class. This shows that a large gap with no occurrences of a class indeed increases labeling errors for that class, and suggests frequent reminders of the concept are needed in a sequence for annotation task.  
% 
We also observed weak significance ($p$-value of 0.11) for the error between the last position and the average of the earlier two positions in the case of annotations for mistake due to potentially unacquired knowledge of the target class. However, it is a major challenge to model the acquisition of knowledge for a concept due to lack of information on the prior knowledge of the annotators.    

Based on these motivating results for the validation of human errors, we next describe large-scale simulations and algorithmic solution to mitigate such human errors focusing on slips due to forgetting.

% \begin{figure}
% \centering
% \includegraphics[scale=0.5]{crowd-exp-sequences-1.png}
% \caption{Illustrative instance sequence with the class labels for the crowdsourcing experiments. The red color indicates the positions of the target class for the error observations shown in table~\ref{tbl:crowd}. \label{fig:sequences}}
% \inote{1. must be readable in black and white; 2. inline in text}
% \vspace{-0.2in}
% \end{figure}
